Deep Learning Aided Laplace Based Bayesian Inference for Epidemiological Systems

Parameter estimation and associated uncertainty quantification is an important problem in dynamical systems characterized by ordinary differential equation (ODE) models that are often nonlinear. Typically, such models have analytically intractable trajectories which result in likelihoods and posterior distributions that are similarly intractable. Bayesian inference for ODE systems via simulation methods require numerical approximations to produce inference with high accuracy at a cost of heavy computational power and slow convergence. At the same time, Artificial Neural Networks (ANN) offer tractability that can be utilized to construct an approximate but tractable likelihood and posterior distribution. In this paper we propose a hybrid approach, where Laplace-based Bayesian inference is combined with an ANN architecture for obtaining approximations to the ODE trajectories as a function of the unknown initial values and system parameters. Suitable choices of a collocation grid and customized loss functions are proposed to fine tune the ODE trajectories and Laplace approximation. The effectiveness of our proposed methods is demonstrated using an epidemiological system with non-analytical solutions, the Susceptible-Infectious-Removed (SIR) model for infectious diseases, based on simulated and real-life influenza datasets. The novelty and attractiveness of our proposed approach include (i) a new development of Bayesian inference using ANN architectures for ODE based dynamical systems, and (ii) a computationally fast posterior inference by avoiding convergence issues of benchmark Markov Chain Monte Carlo methods. These two features establish the developed approach as an accurate alternative to traditional Bayesian computational methods, with improved computational cost.

==> bibfile.tex <==
@article{storvik2002particle,
  title={Particle filters for state-space models with the presence of unknown static parameters},
  author={Storvik, Geir},
  journal={IEEE Transactions on signal Processing},
  volume={50},
  number={2},
  pages={281--289},
  year={2002},
  publisher={IEEE}
}

@article{carvalho2010particle,
  title={Particle learning and smoothing},
  author={Carvalho, Carlos M and Johannes, Michael S and Lopes, Hedibert F and Polson, Nicholas G},
  journal={Statistical Science},
  volume={25},
  number={1},
  pages={88--106},
  year={2010},
  publisher={Institute of Mathematical Statistics}
}

@article{jiang2017learning,
  title={Learning summary statistic for approximate Bayesian computation via deep neural network},
  author={Jiang, Bai and Wu, Tung-yu and Zheng, Charles and Wong, Wing H},
  journal={Statistica Sinica},
  pages={1595--1618},
  year={2017},
  publisher={JSTOR}
}

@article{kermack1927contribution,
	title={A contribution to the mathematical theory of epidemics},
	author={Kermack, William Ogilvy and McKendrick, Anderson G},
	journal={Proceedings of the royal society of london. Series A, Containing papers of a mathematical and physical character},
	volume={115},
	number={772},
	pages={700--721},
	year={1927},
	publisher={The Royal Society London}
}

@article{nguyen1999approximation,
	title={Approximation of functions and their derivatives: A neural network implementation with applications},
	author={Nguyen-Thien, T and Tran-Cong, T},
	journal={Applied Mathematical Modelling},
	volume={23},
	number={9},
	pages={687--704},
	year={1999},
	publisher={Elsevier}
}
@article{mcculloch1943logical,
	title={A logical calculus of the ideas immanent in nervous activity},
	author={McCulloch, Warren S and Pitts, Walter},
	journal={The bulletin of mathematical biophysics},
	volume={5},
	number={4},
	pages={115--133},
	year={1943},
	publisher={Springer}
}

@article{cybenko1989approximation,
	title={Approximation by superpositions of a sigmoidal function},
	author={Cybenko, George},
	journal={Mathematics of control, signals and systems},
	volume={2},
	number={4},
	pages={303--314},
	year={1989},
	publisher={Springer}
}

@article{ferrari2005smooth,
	title={Smooth function approximation using neural networks},
	author={Ferrari, Silvia and Stengel, Robert F},
	journal={IEEE Transactions on Neural Networks},
	volume={16},
	number={1},
	pages={24--38},
	year={2005},
	publisher={IEEE}
}

@article{adcock2021gap,
	title={The gap between theory and practice in function approximation with deep neural networks},
	author={Adcock, Ben and Dexter, Nick},
	journal={SIAM Journal on Mathematics of Data Science},
	volume={3},
	number={2},
	pages={624--655},
	year={2021},
	publisher={SIAM}
}

@article{zainuddin2008function,
	title={Function approximation using artificial neural networks},
	author={Zainuddin, Zarita and Pauline, Ong},
	journal={WSEAS Transactions on Mathematics},
	volume={7},
	number={6},
	pages={333--338},
	year={2008},
	publisher={World Scientific and Engineering Academy and Society (WSEAS)}
}
	
@article{yang2013investigation,
	title={Investigation of neural networks for function approximation},
	author={Yang, Sibo and Ting, TO and Man, Ka Lok and Guan, Sheng-Uei},
	journal={Procedia Computer Science},
	volume={17},
	pages={586--594},
	year={2013},
	publisher={Elsevier}
}
	
@article{li1996simultaneous,
	title={Simultaneous approximations of multivariate functions and their derivatives by neural networks with one hidden layer},
	author={Li, Xin},
	journal={Neurocomputing},
	volume={12},
	number={4},
	pages={327--343},
	year={1996},
	publisher={Elsevier}
}
	
@article{pukrittayakamee2011practical,
	title={Practical training framework for fitting a function and its derivatives},
	author={Pukrittayakamee, Arjpolson and Hagan, Martin and Raff, Lionel and Bukkapatnam, Satish TS and Komanduri, Ranga},
	journal={IEEE transactions on neural networks},
	volume={22},
	number={6},
	pages={936--947},
	year={2011},
	publisher={IEEE}
}
	
@article{lagaris1998artificial,
	title={Artificial neural networks for solving ordinary and partial differential equations},
	author={Lagaris, Isaac E and Likas, Aristidis and Fotiadis, Dimitrios I},
	journal={IEEE transactions on neural networks},
	volume={9},
	number={5},
	pages={987--1000},
	year={1998},
	publisher={IEEE}
}
	
@article{he2000multilayer,
	title={Multilayer neural networks for solving a class of partial differential equations},
	author={He, Shouling and Reif, Konrad and Unbehauen, Rolf},
	journal={Neural networks},
	volume={13},
	number={3},
	pages={385--396},
	year={2000},
	publisher={Elsevier}
}

@proceedings{basson1999approximation,
	title={Approximation of a function and its derivatives in feedforward neural networks},
	author={Basson, E and Engelbrecht, Andries P},
	booktitle={IJCNN'99. International Joint Conference on Neural Networks. Proceedings (Cat. No. 99CH36339)},
	volume={1},
	pages={419--421},
	year={1999},
	organization={IEEE}
}
	
@article{avrutskiy2020enhancing,
	title={Enhancing Function Approximation Abilities of Neural Networks by Training Derivatives},
	author={Avrutskiy, Vsevolod I},
	journal={IEEE transactions on neural networks and learning systems},
	volume={32},
	number={2},
	pages={916--924},
	year={2020},
	publisher={IEEE}
}
	
@article{mai2003approximation,
	title={Approximation of function and its derivatives using radial basis function networks},
	author={Mai-Duy, Nam and Tran-Cong, Thanh},
	journal={Applied Mathematical Modelling},
	volume={27},
	number={3},
	pages={197--220},
	year={2003},
	publisher={Elsevier}
}
	
@article{jianyu2003numerical,
	title={Numerical solution of elliptic partial differential equation using radial basis function neural networks},
	author={Jianyu, Li and Siwei, Luo and Yingjian, Qi and Yaping, Huang},
	journal={Neural Networks},
	volume={16},
	number={5-6},
	pages={729--734},
	year={2003},
	publisher={Elsevier}
}
	
@article{sarra2005adaptive,
	title={Adaptive radial basis function methods for time dependent partial differential equations},
	author={Sarra, Scott A},
	journal={Applied Numerical Mathematics},
	volume={54},
	number={1},
	pages={79--94},
	year={2005},
	publisher={Elsevier}
}
	
@article{gallant1992learning,
	title={On learning the derivatives of an unknown mapping with multilayer feedforward networks},
	author={Gallant, A Ronald and White, Halbert},
	journal={Neural Networks},
	volume={5},
	number={1},
	pages={129--138},
	year={1992},
	publisher={Elsevier}
}

@article{jo2020analysis,
  title={Analysis of COVID-19 spread in South Korea using the SIR model with time-dependent parameters and deep learning},
  author={Jo, Hyeontae and Son, Hwijae and Hwang, Hyung Ju and Jung, Se Young},
  journal={medRxiv},
  year={2020},
  publisher={Cold Spring Harbor Laboratory Press}
}

@article{jo2020deep,
  title={Deep neural network approach to forward-inverse problems},
  author={Jo, Hyeontae and Son, Hwijae and Hwang, Hyung Ju and Kim, Eun Heui},
  journal={Networks \& Heterogeneous Media},
  volume={15},
  number={2},
  pages={247},
  year={2020},
  publisher={American Institute of Mathematical Sciences}
}

@article{raissi2019physics,
  title={Physics-informed neural networks: A deep learning framework for solving forward and inverse problems involving nonlinear partial differential equations},
  author={Raissi, Maziar and Perdikaris, Paris and Karniadakis, George E},
  journal={Journal of Computational Physics},
  volume={378},
  pages={686--707},
  year={2019},
  publisher={Elsevier}
}

@article{ramsay2007parameter,
  title={Parameter estimation for differential equations: a generalized smoothing approach},
  author={Ramsay, Jim O and Hooker, Giles and Campbell, David and Cao, Jiguo},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={69},
  number={5},
  pages={741--796},
  year={2007},
  publisher={Wiley Online Library}
}

@article{hornik1989multilayer,
  title={Multilayer feedforward networks are universal approximators},
  author={Hornik, Kurt and Stinchcombe, Maxwell and White, Halbert},
  journal={Neural networks},
  volume={2},
  number={5},
  pages={359--366},
  year={1989},
  publisher={Elsevier}
}
